Context-Aware Route Planning for Automated Warehouses

In order to ensure efficient flow of goods in an automated warehouse and to guarantee its continuous distribution to/from picking stations in an effective way, decisions about which goods will be delivered to which particular picking station by which robot and by which path and in which time have to be made based on the current state of the warehouse. This task involves solution of two suproblems: (1) task allocation in which an assignment of robots to goods they have to deliver at a particular time is found and (2) planning of collision-free trajectories for particular robots (given their actual and goal positions). The trajectory planning problem is addressed in this paper taking into account specifics of automated warehouses. First, assignments of all robots are not known in advance, they are instead presented to the algorithm gradually one by one. Moreover, we do not optimize a makespan, but a throughput - the sum of individual robot plan costs. We introduce a novel approach to this problem which is based on the context-aware route planning algorithm [1]. The performed experimental results show that the proposed approach has a lower fail rate and produces results of higher quality than the original algorithm. This is redeemed by higher computational complexity which is nevertheless low enough for real-time planning.

==> experiments_old_.tex <==
\section{Experiments}
\label{sec:exp}

The experiments were performed on a computer equiped with Intel Xeon E5-2690.
The maps the experiments were performed on were created to show how the proposed algorithm performs depending on the density of the given graph, specifically the number of edges.
The set of 21 maps was generated by creating a minimum spanning tree of a 20x20 grid map and then iteratively adding a set number of  original edges to it untill the original grid was recreated.
Furthermore, 500 different random assignments gere generated for a fleet of 100 robots by randomly sampling start and goal nodes for each robot.
Each of these assignments was tested on all 21 maps.

The configuration of algorithms was as follows: CARP algorithm was tested in CARP, CARP10, CARP100 and CARP1000 that ran the the CARP algorithm on set of robot priorities that was randomly shuffled 0,10,100 and 1000 times respectively.
A set of prioroties assigned by the longest first rule was also tested as CARPordered.
Our one cluster approach was tested using cluster sizes 4 and 5 and can be seen in the results as $OneCluster_l4$ and $OneCluster_l5$ respectively.




\begin{figure*}[htb]
\begin{tabular}{cc}
\includegraphics[width=\columnwidth]{./imgs/fails.png} &
\includegraphics[width=\columnwidth]{./imgs/length.png} \\

\includegraphics[width=\columnwidth]{./imgs/longest.png} &
\includegraphics[width=\columnwidth]{./imgs/makespan.png} \\

\includegraphics[width=\columnwidth]{./imgs/time.png} &
\includegraphics[width=\columnwidth]{./imgs/time_one.png} \\
 
\end{tabular}
\caption{Results of the experiment}
\label{fig:first_experiment}
\end{figure*}
